Unsupervised Recycled FPGA Detection Using Symmetry Analysis

Recently, recycled field-programmable gate arrays (FPGAs) pose a significant hardware security problem due to the proliferation of the semiconductor supply chain. Ring oscillator (RO) based frequency analyzing technique is one of the popular methods, where most studies used the known fresh FPGAs (KFFs) in machine learning-based detection, which is not a realistic approach. In this paper, we present a novel recycled FPGA detection method by examining the symmetry information of the RO frequency using unsupervised anomaly detection method. Due to the symmetrical array structure of the FPGA, some adjacent logic blocks on an FPGA have comparable RO frequencies, hence our method simply analyzes the RO frequencies of those blocks to determine how similar they are. The proposed approach efficiently categorizes recycled FPGAs by utilizing direct density ratio estimation through outliers detection. Experiments using Xilinx Artix-7 FPGAs demonstrate that the proposed method accurately classifies recycled FPGAs from 10 fresh FPGAs by x fewer computations compared with the conventional method.

==> tex/related.tex <==
%\section{Related Works Discussion}\label{sec:related}
\section{{\shintani{Preliminary}}}\label{sec:related}
\subsection{{\shintani{Recycled FPGA detection}}}

\begin{figure}[!t]
  \centering
  \includegraphics[clip, width=0.65\linewidth]{fig/flow.pdf}
  \caption{Flow of the conventional recycled FPGA detection~\cite{R_FPGA}.}
  \label{fig:conv_flow}
\end{figure}

% If necessary, principle component analysis (PCA) is conducted to
% reduce the feature vector for the effective machine learning
% classification.

{\shintani{
The flow of the recycled FPGA detection proposed in~\cite{R_FPGA} is
depicted in Fig.~\ref{fig:conv_flow}. In~\cite{R_FPGA}, the existence
of golden FPGAs is assumed. The flow consists of the following three
steps. (1) Multiple ROs are designed on all the golden FPGAs and
measured to use the frequencies as feature vector of the following
machine learning.  The recycled FPGA detection is formulated as an
outlier detection problem to classify FPGA under test (FUT) into fresh
or aged FPGAs.
% , and then a database of the frequencies is constructed.
The machine-learning algorithm {\michiko{trains a model}} using the
frequencies. Here, if the feature vector size is too large to converge the
training, principle component analysis (PCA) is conducted to reduce the
feature size. (2) On the user side, before an FUT is
implemented into system, frequencies of ROs are measured as with step
(1). Then, the measured data is sent to the manufacture to query whether the
FUT is fresh or not.  (3) {\michiko{The frequencies obtained in step (2) are
    applied to the trained model to test}} whether the FUT is fresh or {\foisal{recycled}}. If the FUT is previously used, some RO frequencies will degrade due to
the aging mechanism, such as negative bias temperature instability
(NBTI)~\cite{CICC2006_Bhardwaj}. As a result, the recycled FPGAs can be
detected through the machine-learning-based classification.}}

% As the RO, a simple inverter-based RO is used in~\cite{R_FPGA}.
% Fingerprinting FPGA technique of~\cite{R_FP} is also
% {\foisal{followed by}} the concept of~\cite{R_FPGA} and it is an
% effective way to detect recycled FPGAs in supply
% chain. In~\cite{R_FP}, the fingerprints of the fresh ones are stored
% into the golden FPGA database before shipping.}}

% Figure~\ref{fig:fpga} shows the general architecture of FPGA. The
% discussion of the internal architecture of the FPGA is important to
% describe the previous works properly. Basically, FPGA is composed of
% an array of configurable logic blocks (CLBs) and programmable logic
% switches with interconnections. FPGAs can implement any logic
% functions by appropriately configuring the look-up tables (LUTs) which
% are basically built of SRAM and a set of multiplexers (MUX) to select
% the SRAM bit into the corresponding output path. FPGA manufacturer
% company does not disclose the circuit level of
% LUTs. Figure~\ref{fig:fpga} simply shows transmission gate based
% implementation of the 2-input LUTs structure as an example. By
% connecting multiple LUTs, multiple stages ROs can be designed.

{\shintani{
The two methods of~\cite{R_FP,R_ITC} are also based on the concept
of~\cite{R_FPGA} where RO-based measurements are conducted for the golden FPGAs
in order to detect the recycled FPGA.
% using one-class SVM machine learning algorithm~\cite{R_onesvm}.
In~\cite{R_FPGA}, only a few paths of LUTs in the FPGAs are covered in
recycled detection.
% As shown from the Fig.~\ref{fig:fpga}, the 2-input LUTs have total three
% paths since one of the inputs is used to form a stage of the RO.
Thus, any of the other paths may have the possibility of the aging
degradation which idea is highlighted as exhaustively characterizing
all the paths in several LUTs~\cite{R_ITC}. However, they analyzed only
few parts of the total LUTs while other parts of the LUTs in the FPGA
may be aged. In~\cite{R_FP}, consider all part of the entire
location of the LUTs where an FP of each FPGA is obtained to represent
a unique spatial process variation in recycled FPGA
detection. By contrast, other paths of the LUTs are not analyzed in the
detection.}}

%{\shintani{
%In order to accurately characterize the frequencies,
{\camera{We would like to note that the RO characterization should be conducted one
by one to avoid power or signal interference from other ROs. It is hence
obvious that the detection accuracy at the classification highly
depends on the number of the ROs.}} While the volume of
the measurement data must be sufficient in order to effectively
classify the FUTs, the additional measurement cost is imposed on the
manufacturer.  In this work, VP technique is utilized to reduce the
number of the RO measurements.

\subsection{{\shintani{Virtual Probe Technique}}}
\input{./tex/vp.tex}


==> tex/vp.tex <==
{\shintani{
VP is a technique based on compressed sensing and has been originally
developed for a low-cost wafer-level silicon characterization~\cite{R_VP2}.
% The key concept of the VP technique is to predict the performance of all
% chips on a wafer from the small sample chip measurement.
In the VP technique, a subset {\michiko{of}} chips randomly selected on a wafer and tested,
then the performances of the other chips are predicted through a statistical
algorithm using the information from the tested chips.}}

{\shintani{
We denote $g(x,y)$ as the two-dimensional function of the performance metric
$g$, such as frequency, resistance, and leakage current, where $x$ and $y$
are the position coordinate on a wafer and labeled as $x \in \{1,2,\cdots,P\}$
and $y \in \{1,2,\cdots,Q\}$.  The relationship between the performance metric
and its frequency-domain component can be written by discrete cosine
transform (DCT) as follows:
\begin{eqnarray}
  G(u,v)&=\sum^P_{x=1} \sum^Q_{y=1} \alpha_u \cdot \beta_v \cdot g(x,y)
          \nonumber \\ &\cdot \cos \frac{\pi(2x-1)(u-1)}{2P}
                         \cdot \cos \frac{\pi(2y-1)(v-1)}{2Q},
\end{eqnarray}
where
\begin{eqnarray}
\alpha_u = \left\{
                \begin{array}{ll}
                  \sqrt{(1/P)}\quad (u=1)\\
                  \sqrt{(2/P)}\quad (2\leq u \leq P)
                \end{array}
              \right.\\
\beta_v = \left\{
                \begin{array}{ll}
                  \sqrt{(1/Q)}\quad (v=1)\\
                  \sqrt{(2/Q)}\quad (2\leq v \leq Q).
                \end{array}
              \right.
\end{eqnarray}
Here, $ G(u,v)$ represents the DCT coefficients, where $u {\michiko{\in}} \{1,2,\cdots,P\}$
and $v {\michiko{\in}} \{1,2,\cdots,Q\}$. Equivalently, using inverse discrete cosine
transform (IDCT), $g(x,y)$ can be represented as a linear combination as:
\begin{eqnarray}
  g(x,y)&=\sum^P_{u=1} \sum^Q_{v=1} \alpha_u \cdot \beta_v \cdot G(u,v)
          \nonumber \\ &\cdot \cos \frac{\pi(2x-1)(u-1)}{2P}
                         \cdot \cos \frac{\pi(2y-1)(v-1)}{2Q}.
\label{eq:4}
\end{eqnarray}
}}
% Similarly, the original sampled values can be
% recovered by the inverse discrete cosine transform (IDCT).

{\shintani{
Generally, it is trivial to uniquely determine the $g(x,y)$, once the DCT
coefficients $ G(u,v)$ are known and vice versa. This problem can be
mathematically constructed by a linear equation as follows:
\begin{eqnarray}
  \bm{A} \cdot \bm{s}= \bm{y},
  \label{eq:5}
\end{eqnarray}
where
\begin{eqnarray}
  \bm{A}=\begin{bmatrix}
    A_{1,1,1} & A_{1,1,2} & A_{1,1,3} & \dots  & A_{1,P,Q} \\
    A_{2,1,1} & A_{2,1,2} & A_{2,1,3} & \dots  & A_{2,P,Q} \\
    \vdots & \vdots & \vdots & \ddots & \vdots \\
    A_{M,1,1} & A_{M,1,2} & A_{M,1,3} & \dots  & A_{M,P,Q}
\label{eq:matrix-A}
\end{bmatrix},
\end{eqnarray}
\begin{eqnarray}
  A_{m,u,v}&=\alpha_u \cdot \beta_v \cdot \cos \frac{\pi(2x_m-1)(u-1)}{2P}
             \nonumber\\&\cdot \cos \frac{\pi(2y_m-1)(v-1)}{2Q},
\end{eqnarray}
\begin{eqnarray}
  \bm{s}=[G(1,1)\quad G(1,2)\quad \cdots\quad G(P,Q)]^T,
\end{eqnarray}
and
\begin{eqnarray}
  \bm{y}=[g(x_1,y_1)\quad g(x_2,y_2)\quad \cdots \quad g(x_M,y_M)]^T.
  \label{eq:9}
\end{eqnarray}
}}{\shintani{In order to derive $g(x,y)$, the DCT coefficients
  $\bm{s}$ need to be determined using Eqs.~(\ref{eq:5})
  to~(\ref{eq:9}). However, it is not easy task {\michiko{if}}
  Eq.~(\ref{eq:5}) is an under-determined linear equation, {\michiko{that is,}} the
  number of samples $M$, taken at some locations
  $\{(x_m,y_m);\,m=1,2,\cdots, M\}$, is {\michiko{much smaller}} than $PQ$, i.e., $M \ll PQ$.
%  According to the VP technique~\cite{R_VP2},
  %% the sampling values $g(x,y)$ can be accurately recovered with a very small
  %% number of samples, e.g. $M$, taken at some locations
  %% $\{(x_m,y_m);\,m=1,2,\cdots, M\}$, where .  In order to solve the
  The VP technique assumes that the solution $\bm{s}$ is
  sparse~\cite{R_VP2}. As the systematic component of the process
  variation gradually changes over a wafer, the high frequency
  components of the DCT coefficients are close to zero, thus the
  sparse representation assumption is reasonably supported in the
  wafer-level characterization.  In order to find the sparse
  solution of $\bm{s}$, the following optimization problem is
  formulated as:
\begin{equation}
\begin{aligned}
& \underset{\bm{s}}{\text{minimize}}
& & \left\Vert \bm{s} \right\Vert_1 \\
& \text{subject to}
& & \bm{A} \cdot \bm{s} = \bm{y},
\label{eq:14}
\end{aligned}
\end{equation}
where $\left\Vert \bm{s} \right\Vert_1$ is the $L_1$-norm of a vector. Using
convex optimization and linear programming, the feasible sparse solution can
be obtained from Eq.~(\ref{eq:14}). Although, the $L_0$-norm
provides more accurate solution instead of the $L_1$-norm, the optimization
problem for the $L_0$-norm is NP hard and hence the $L_1$-norm is used to
solve it within a practical time in the VP technique.  Finally, once the DCT
coefficients $\bm{s}$ are obtained, the $\hat{g}(x,y)$, which is the
{\foisal{prediction of}} $g$ at $(x,y)$, can be calculated by IDCT as in
Eq.~(\ref{eq:4}). }}

% In the MAP algorithm, VP technique used zero-mean Laplace
% distribution to predict the prior distribution for $s$ as the probability
% density function (PDF) of {$s_i=1,2,.....,PQ$}:
% \begin{eqnarray}
% pdf(s_i)=\frac{1}{2\lambda}\cdot \exp\bigg(-\frac{\abs{s_i}}{\lambda}\bigg)\quad
% (i=1,2,.....,PQ)
% \label{eq:10}
% \end{eqnarray}
% where $pdf(s_i)$ denotes as the PDF of $s_i$ and $\lambda$ is a
% independent parameter that controls the variance of PDF
% distribution. After considering all DCT coefficients as mutually
% independent in the vector $s\,\epsilon\,R^{PQ}$, the Eq.~\eqref{eq:10}
% further represented by the joint PDF of $s$ as:
% \begin{eqnarray}
% pdf(s)=\Big(\frac{1}{2\lambda}\Big)^{PQ}\cdot \exp\bigg(-\frac{\left\Vert
% s \right\Vert_1 }{\lambda}\bigg)
% \label{eq:11}
% \end{eqnarray}
% where $ \left\Vert s \right\Vert_1 $ is the $L_1-$norm which means the
% summation of the absolute value of all elements in $s$.

% The main idea behind the MAP algorithm is to find the optimal solution
% of $s$ that maximizes the posterior distribution in Bayes'
% theorem~\cite{R_PAT}. According to Bayes' theorem, posterior
% distribution $pdf(s\mid A\cdot s=y)$ is directly proportional to the
% prior distribution $pdf(s)$ and the likelihood function $pdf(A\cdot
% s=y\mid s)$ as:
% \begin{eqnarray}
% pdf(s\mid A \cdot s=y)\propto pdf(s)\cdot pdf(A\cdot s = y \mid s)
% \label{eq:12}
% \end{eqnarray}
% For the likelihood function, Dirac delta function is used in VP
% technique and hence, maximizing the posterior probability in
% Eq.~\eqref{eq:12} can be represented further as:
% \begin{equation}
% \begin{aligned}
% & \underset{s}{\text{maximize}} &
% & \frac{1}{(2\lambda)^{PQ}}\cdot \exp\bigg(-\frac{\left\Vert
% s \right\Vert_1 }{\lambda}\bigg) \\ & \text{subject to} & & A\cdot s =
% y
% \label{eq:13}
% \end{aligned}
% \end{equation}

% As the exponential function $\exp(-\left\Vert s \right\Vert_1
% / \lambda)$ decreases monotonically with $\lambda >0$, the optimization
% problem in Eq.~\eqref{eq:13} can be further represented as:
% \begin{equation}
% \begin{aligned}
% & \underset{s}{\text{minimize}}
% & & \left\Vert s \right\Vert_1 \\
% & \text{subject to}
% & & A\cdot s = y
% \label{eq:14}
% \end{aligned}
% \end{equation}
% The Eq.~\eqref{eq:14} is a $L_1-norm$ regularization problem. Using convex
% optimization and linear programming method, the feasible unique solution can
% be obtained in a near polynomial time. Once the DCT coefficients $s$ are
% obtained, the original function $g(x,y)$ can be reconstructed by IDCT as in
% Eq.~\eqref{eq:4}.

% We discuss the basic idea of compressed sensing (CS) upon
% which VP algorithm is developed.
% The idea of CS is one of the important revolutions in the signal processing
% and statistics field after the invention of well known Nyquist
% criterion~\cite{R_CS1,R_CS2}.
% The main difference between the VP and CS is the number of samples required
% to represent the signal. The sampling rate of the Nyquist criterion is the
% twice of the maximum number of frequency, whereas, in the CS technique, it
% is controlled by the signal sparsity~\cite{R_CS6}. The signal is possible to
% make compressed if it has some kind of sparsity properties as seen in many
% natural and man-made signal like images, speech etc. For example, the speech
% signal and many communication signals can be compressed by Fourier transform
% and natural images can be represented using a wavelet domain or discrete
% cosine transform (DCT) in a JPEG compression
% standard~\cite{R_wavelet}. However, all of the compression techniques, the
% first step is to collect the total number of samples based on the Nyquist
% criterion and then compress, which eventually experiences significant time
% and cost. On the other hand, in CS measurement instead of taking all $N$
% number of samples, it measures only a few numbers of M ($M \ll N$) samples
% in the measurement steps.
% as shown in Fig.~\ref{fig:cs_measurement}.

% The idea of CS is one of the important revolutions in the signal processing
% and statistics field after the invention of well known Nyquist
% criterion~\cite{R_CS1,R_CS2}. The main difference between the two methods is
% the number of samples required to represent the signal. The sampling rate of
% the Nyquist criterion is the twice of the maximum number of frequency,
% whereas, in the CS technique, it is controlled by the signal
% sparsity~\cite{R_CS6}. The signal is possible to make compressed if it has
% some kind of sparsity properties as seen in many natural and man-made signal
% like images, speech etc. For example, the speech signal and many
% communication signals can be compressed by Fourier transform and natural
% images can be represented using a wavelet domain or discrete cosine
% transform (DCT) in a JPEG compression standard~\cite{R_wavelet}. However,
% all of the compression techniques, the first step is to collect the total
% number of samples based on the Nyquist criterion and then compress, which
% eventually experiences significant time and cost. On the other hand, in CS
% measurement instead of taking all N number of samples, it measures only a
% few numbers of M ($M \ll N$) samples in the measurement steps as shown in
% Fig.~\ref{fig:cs_measurement}.

% \begin{figure}[!t]
%   \centering
%   \subfigure[Compressed measurement]{
%     \includegraphics[width=0.7\linewidth]{fig/cs_measurement.pdf}
%     \label{fig:cs_measurement}
%   }
%   \hspace{-3mm}
%   \subfigure[Recovery]{
%     \includegraphics[width=0.7\linewidth]{fig/cs_recover.pdf}
%     \label{fig:cs_recover}
%   }
%   \caption{Basic compressed sensing steps.}
%   \label{fig:CS}
% \end{figure}

% Figure~\ref{fig:CS} presents the basic steps of the measurement and recovery
% model used in the CS method. In the measurement system, a few number of $M$
% measurements are taken randomly instead of taking all $N$ samples where
% $M \ll N$ and the input signal is $x \in R^N $ of length $N$ can be
% represented in terms of basis of $N\times1$ vectors ${\Psi}^{N}_{i=1} $
% which further make $ N \times N$ basis matrix and are expressed as:
% $x = \sum_{i=1}^{N} \Psi_i s_i = \Psi s$.

% Now, the measurement vector can be represented by stacking all
% measurement data into random measurement matrix ${\Phi}^M_{j=1} \in
% R^{M \times N}$ and the sparse signal shown in
% Fig.~\ref{fig:measure_process}. Thus, this linear compressive
% measurement can be written as~\cite{CS_notes}:
% \begin{eqnarray}
%   y &= \Phi x = \Phi \Psi s= A\cdot s,
%    \label{eq:1}
% \end{eqnarray}
% where $A\in R^{M \times N}$ is the effective measurement matrix and $s$ is the
% sparse representation of the signal of $N \times 1$. The main
% challenge of optimal recovery of the signal \={x} in
% Fig.~\ref{fig:cs_recover} is to design a random measurement matrix A
% and a reconstruction algorithm for K-sparse signal which is totally
% underdetermined linear Eq.~\eqref{eq:1}.

% \begin{figure}[!t]
%   \centering
%   \includegraphics[clip, width=0.5\linewidth]{fig/measure_process.pdf}
%   \caption{Compressed sensing measurement process with random
%     measurement matrix and sparse representation of the signal (K=3).}
%   \label{fig:measure_process}
% \end{figure}
% The original reconstructed signal $\overline{\text x}$ can be
% recovered only by solving the underdetermined linear
% Eq.~\eqref{eq:1}. There is an infinite number of possible
% solutions. However, after rigorously mathematical analysis on the
% convex optimization and linear programming, the feasible unique
% solution can be obtained by solving the L1-norm minimization problem
% in a near polynomial time. The optimization problem in
% Eq.~\eqref{eq:1} can be formulated as~\cite{CS_notes}:
% \begin{eqnarray}
%   \begin{aligned}
%   \overline{x}&=\Psi \overline{s}\\
%   \overline{s}&=\argmin_{s} & \left\Vert s \right\Vert_1 \quad\textrm{s.t.} \quad & \bm{A}\cdot s=y,
%   \label{eq:2}
%   \end{aligned}
% \end{eqnarray}
% where, $\left\Vert s \right\Vert_1$ is known as L1-norm of $s$. The
% estimated value of $\overline{x}$ can be obtained after taking the
% inverse transform of $\overline{s}$ which is the actual sparse
% representation of $\overline{x}$.

% In our proposed method, we have used VP algorithm~\cite{R_VP2} which mainly
% concentrated on the silicon characterizations to exploit the spatial process
% variation using the above compressed sensing technique. Using DCT transform,
% the recovery problem of $\bm{A} \cdot s= y $ is formulated in the proposed VP
% framework. According to the VP method, to increase the estimation of the
% sparse signal for the underdetermined system~\eqref{eq:1}, a column
% normalization technique is applied to improve the orthogonality of the
% matrix $A$ before applying the L1-norm regularization problem. In addition,
% as also mentioned earlier that using M-LHS scheme in VP method, the
% selecting of the spatial sampling location is considered to reduce the
% coherency of the random matrix $A$ in order to enhance the MAP estimation.

